From Batch to Stream: Automatic Generation of Online Algorithms

Online streaming algorithms, tailored for continuous data processing, offer substantial benefits but are often more intricate to design than their offline counterparts. This paper introduces a novel approach for automatically synthesizing online streaming algorithms from their offline versions. In particular, we propose a novel methodology, based on the notion of relational function signature (RFS), for deriving an online algorithm given its offline version. Then, we propose a concrete synthesis algorithm that is an instantiation of the proposed methodology. Our algorithm uses the RFS to decompose the synthesis problem into a set of independent subtasks and uses a combination of symbolic reasoning and search to solve each subproblem. We implement the proposed technique in a new tool called Opera and evaluate it on over 50 tasks spanning two domains: statistical computations and online auctions. Our results show that Opera can automatically derive the online version of the original algorithm for 98% of the tasks. Our experiments also demonstrate that Opera significantly outperforms alternative approaches, including adaptations of SyGuS solvers to this problem as well as two of Opera's own ablations.

==> algo-complete-hole.tex <==
\begin{figure}[!t]
\begin{algorithm}[H]
\caption{Expression synthesis}
\label{algo:complete-hole}
\begin{algorithmic}[1]
\Procedure{\textsc{SynthesizeExpr}}{$\rfs, E$}
\vspace{2pt}
\Statex \textbf{Input:} Relational function signature $\rfs$, offline expression $E$
\Statex \textbf{Output:} Online expression $E'$
%\State $r \gets \textsf{FacreshVar}(), x \gets \textsf{FreshVar}()$
%\State $\psi_1 \gets \textsf{Encode}(r = E[ (xs \listappend [x]) / xs])$
%\State $\psi_2 \gets \textsf{Encode}(\rfs)$
%\State $\psi \gets \textsf{QE}(xs, \psi_1 \land \psi_2)$
\State $T \gets \textsc{FindImplicates}(\rfs, E[xs\pp[x]/xs] = \hole)$
\State $G \gets \textsf{AddTermsToGrammar}(T)$
\State \Return $\textsf{EnumSynthesis}(G, E, \rfs)$
\vspace{2pt}
\EndProcedure

\Procedure{\textsc{FindImplicates}}{$\rfs, E$}
\vspace{2pt}
\Statex \textbf{Input:} Relational function signature $\rfs$, offline expression $E$
\Statex \textbf{Output:} Online expression $E'$
%\State $r \gets \textsf{FreshVar}(), x \gets \textsf{FreshVar}()$
%\State $\psi_1 \gets \textsf{Encode}(r = E[ (xs \listappend [x]) / xs])$
%\State $\psi_2 \gets \textsf{Encode}(\rfs)$
%\State $\psi \gets \textsf{QE}(xs, \psi_1 \land \psi_2)$
\State $T \gets \textsc{FindImplicates}(\rfs, E[xs\pp[x]/xs] = \hole)$
\State $G \gets \textsf{AddTermsToGrammar}(T)$
\State \Return $\textsf{EnumSynthesis}(G, E, \rfs)$
\vspace{2pt}
\EndProcedure
\end{algorithmic}
\end{algorithm}
\end{figure}


==> algo-gen-sketech.tex <==
\begin{figure}[!t]
\begin{algorithm}[H]
\caption{Sketch Generation}
\label{algo:gen-sketch}
\begin{algorithmic}[1]
\Procedure{\textsc{GenSketech}}{$\rfs, \prog$}
\vspace{2pt}
\Statex \textbf{Input:} Relational function signature $\rfs$, offline program $\prog$
\Statex \textbf{Output:} A sketch $\sketch$ with $\context$ mapping each hole to the corresponding offline expression
\State $\sketch \gets (y_1, \ldots, y_n)$ where $y_1, \ldots, y_n \in \dom(\rfs)$
\For{$v \in \dom(\rfs)$}
    \State $\sketch \gets \sketch[\rfs[v] / v]$
\EndFor
\State $\context \gets \set{}$
\For{\textbf{each} $E \in \textsf{PrimitiveStreamExprs}(\sketch)$}
    \State $h \gets \textsf{FreshHole}()$
    \State $\sketch \gets \sketch[h/E]$
    \State $\context \gets \context[h \mapsto E]$
\EndFor
\State \Return $\sketch, \context$
\vspace{2pt}
\EndProcedure
\end{algorithmic}
\end{algorithm}
\end{figure}


==> fig-scheme-semantics.tex <==
\begin{figure}[!t]
\[
\begin{array}{c}
\irulelabel
{}
{\denot{(I, P)}_{\nil} = \nil}
{\textrm{(Lift-Nil)}}

\irulelabel
{\begin{array}{c}
    \denot{P}_{h, I} = c \quad
    t, c \vdash (I, P) \Downarrow s
\end{array}}
{\denot{(I, P)}_{h:t} = \fst(c) : s}
{\textrm{(Lift-Cons)}}

\\ \ \\

\irulelabel
{}
{\nil, \_ \vdash (I, P) \Downarrow \nil}
{\textrm{(S-Nil)}}

\irulelabel
{\begin{array}{c}
    \denot{P}_{h, c} = c' \quad
    t, c' \vdash (I, P) \Downarrow s
\end{array}}
{h:t, c \vdash (I, P) \Downarrow \fst(c') : s}
{\textrm{(S-Cons)}}

\end{array}
\]
\caption{Semantics of the online scheme. $\denot{(I, P)}_s = s'$ means evaluating online scheme $(I, P)$ on stream $s$ yields stream $s'$, and $s, c \vdash (I, P) \Downarrow s'$ is an auxiliary relation, meaning online scheme $(I, P)$ evaluates to $s'$ given stream $s$ and current accumulators $c$.}
\label{fig:scheme-semantics}
\end{figure}


==> pics/ablation-cdf.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{forestgreen4416044}{RGB}{44,160,44}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{axis}[
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.97,0.03)},
  anchor=south east,
  draw=lightgray204
},
tick align=outside,
tick pos=left,
title={Number of Benchmarks Solved by Time},
x grid style={darkgray176},
xlabel={Running Total (sec)},
xmajorgrids,
xmin=0, xmax=250,
xtick style={color=black},
y grid style={darkgray176},
ylabel={# of Benchmarks Solved},
ymajorgrids,
ymin=0, ymax=100,
ytick style={color=black}
]
\path [draw=steelblue31119180, fill=steelblue31119180, opacity=0.2]
(axis cs:10000000000,91.3165266106443)
--(axis cs:10000000000,83.0532212885154)
--(axis cs:10000000000,91.3165266106443)
--(axis cs:10000000000,91.3165266106443)
--cycle;

\path [draw=forestgreen4416044, fill=forestgreen4416044, opacity=0.2]
(axis cs:10000000000,89.042675893887)
--(axis cs:10000000000,79.8154555940023)
--(axis cs:10000000000,89.042675893887)
--(axis cs:10000000000,89.042675893887)
--cycle;

\addplot [semithick, steelblue31119180, mark=*, mark size=3, mark options={solid,draw=white}, forget plot]
table {%
0.117 1.96078431372549
0.134 3.92156862745098
0.143 5.88235294117647
0.145 7.84313725490196
0.222 9.80392156862745
0.238 11.7647058823529
0.313 13.7254901960784
0.335 15.6862745098039
0.356 17.6470588235294
0.358 19.6078431372549
0.376 21.5686274509804
0.384 23.5294117647059
0.521 25.4901960784314
0.639 27.4509803921569
0.857 29.4117647058824
0.969 31.3725490196078
0.97 33.3333333333333
1.405 35.2941176470588
1.407 37.2549019607843
1.995 39.2156862745098
2.77 41.1764705882353
2.992 43.1372549019608
3.723 45.0980392156863
4.177 47.0588235294118
4.2 49.0196078431373
5.17 50.9803921568627
5.414 52.9411764705882
6.775 54.9019607843137
7.526 56.8627450980392
7.759 58.8235294117647
16.645 60.7843137254902
21.952 62.7450980392157
29.117 64.7058823529412
29.662 66.6666666666667
38.2 68.6274509803922
62.75 70.5882352941177
116.187 72.5490196078431
};
\addplot [semithick, darkorange25512714, mark=x, mark size=3, mark options={solid,draw=white}, forget plot]
table {%
0.18 1.96078431372549
0.211 3.92156862745098
0.221 5.88235294117647
0.335 7.84313725490196
0.858 9.80392156862745
0.949 11.7647058823529
0.969 13.7254901960784
0.97 15.6862745098039
0.974 17.6470588235294
1.366 19.6078431372549
1.407 21.5686274509804
1.471 23.5294117647059
1.571 25.4901960784314
1.736 27.4509803921569
1.923 29.4117647058824
1.995 31.3725490196078
2.77 33.3333333333333
2.992 35.2941176470588
3.392 37.2549019607843
3.432 39.2156862745098
3.723 41.1764705882353
3.803 43.1372549019608
3.909 45.0980392156863
4.177 47.0588235294118
5.17 49.0196078431373
5.414 50.9803921568627
7.085 52.9411764705882
7.237 54.9019607843137
7.526 56.8627450980392
7.759 58.8235294117647
12.354 60.7843137254902
14.276 62.7450980392157
16.645 64.7058823529412
21.952 66.6666666666667
29.117 68.6274509803922
29.662 70.5882352941177
32.429 72.5490196078431
32.56 74.5098039215686
32.743 76.4705882352941
38.2 78.4313725490196
50.171 80.3921568627451
62.256 82.3529411764706
67.308 84.3137254901961
68.465 86.2745098039216
76.729 88.2352941176471
77.254 90.1960784313726
84.405 92.156862745098
92.875 94.1176470588235
156.363 96.078431372549
167.579 98.0392156862745
};
\addplot [semithick, forestgreen4416044, forget plot]
table {%
0.335 1.96078431372549
0.336 3.92156862745098
0.969 5.88235294117647
0.97 7.84313725490196
1.407 9.80392156862745
1.811 11.7647058823529
1.83 13.7254901960784
1.995 15.6862745098039
2.54 17.6470588235294
2.77 19.6078431372549
2.992 21.5686274509804
3.015 23.5294117647059
3.723 25.4901960784314
4.177 27.4509803921569
4.627 29.4117647058824
4.897 31.3725490196078
5.17 33.3333333333333
5.414 35.2941176470588
7.526 37.2549019607843
7.759 39.2156862745098
15.609 41.1764705882353
16.645 43.1372549019608
18.081 45.0980392156863
21.952 47.0588235294118
29.117 49.0196078431373
29.662 50.9803921568627
38.2 52.9411764705882
53.093 54.9019607843137
63.51 56.8627450980392
107.724 58.8235294117647
118.049 60.7843137254902
145.296 62.7450980392157
156.409 64.7058823529412
216.052 66.6666666666667
};
\end{axis}

\end{tikzpicture}

